On the Implementation of Dynamic Patterns

The evaluation mechanism of pattern matching with dynamic patterns is modelled in the Pure Pattern Calculus by one single meta-rule. This contribution presents a refinement which narrows the gap between the abstract calculus and its implementation. A calculus is designed to allow reasoning on matching algorithms. The new calculus is proved to be confluent, and to simulate the original Pure Pattern Calculus. A family of new, matching-driven, reduction strategies is proposed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{E. Bonelli (Ed.): 5th International Workshop\\
on Higher-Order Rewriting (HOR'10)\\
EPTCS 49, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.49.2}{10.4204/EPTCS.49.2}}
\pdfoutput=1

